OnSET: Ontology and Semantic Exploration Toolkit

Retrieval over knowledge graphs is usually performed using dedicated, complex query languages like SPARQL. We propose a novel system, Ontology and Semantic Exploration Toolkit (OnSET) that allows non-expert users to easily build queries with visual user guidance provided by topic modelling and semantic search throughout the application. OnSET allows users without any prior information about the ontology or networked knowledge to start exploring topics of interest over knowledge graphs, including the retrieval and detailed exploration of prototypical sub-graphs and their instances. Existing systems either focus on direct graph explorations or do not foster further exploration of the result set. We, however, provide a node-based editor that can extend on these missing properties of existing systems to support the search over big ontologies with sub-graph instances. Furthermore, OnSET combines efficient and open platforms to deploy the system on commodity hardware.

==> figures/erl_constrained.tex <==
\usetikzlibrary {arrows.meta, graphs, shapes.misc, matrix, quotes, patterns, shapes.arrows, shapes.misc, positioning, calc, fit, bending}

\begin{tikzpicture}[
                scale=\erlsize, transform shape,
                entity/.style={rectangle, draw=black!90,  fill=black!20, minimum size=1cm,  text width=1.5cm, font={\Large}, align=center},
                every edge/.append style ={
                                inner sep=0pt, auto,
                                align=left},
                every new --/.style={line width=0.5pt},
        ]
        \node (company) [entity] {company};
        \node (bel_company) [below=of company]{};
        \node (person) [entity, right=3cm of bel_company] {person};
        \node (bel_person) [below=of person]{};
        \node (place) [entity, right=3cm of bel_person, draw=red] {place};
        \graph [use existing nodes] {
        company.east --[ out=0,in=180, draw=red ]person.west;
        person.east--[out=0,in=180]place.west;
        };

\end{tikzpicture}

==> figures/erl_edit.tex <==
\usetikzlibrary{patterns,shapes.arrows}
\usetikzlibrary {arrows.meta, graphs, shapes.misc, matrix, quotes, patterns, shapes.arrows, shapes.misc, positioning, calc, fit, bending}

\begin{tikzpicture}[
                scale=\erlsize, transform shape,
                entity/.style={rectangle, draw=black!90,  fill=black!20, minimum size=1cm,  text width=1.5cm, font={\Large}, align=center},
                every edge/.append style ={
                                inner sep=0pt, auto,
                                align=left},
                every new --/.style={line width=0.5pt},
        ]
        \node (company) [entity] {company};
        \node (person) [entity, right=1.25cm of company] {person};
        \node (bel_person) [below=of person]{};
        \node (place) [entity, right=2cm of bel_person] {place};
        \node (school) [entity, right=1.25cm of person, draw=OliveDrab, fill=OliveDrab!10] {school};
        \graph [use existing nodes] {
        company.east --[ out=0,in=180]person.west;
        person.east--[out=0,in=180]place.west;
        person.east--[out=0,in=180, draw=OliveDrab]school.west;
        };

\end{tikzpicture}

==> figures/erl_ex.tex <==
\usetikzlibrary{patterns,shapes.arrows}
\usetikzlibrary {arrows.meta, graphs, shapes.misc, matrix, quotes, patterns, shapes.arrows, shapes.misc, positioning, calc, fit, bending}

\begin{tikzpicture}[
                scale=\erlsize, transform shape,
                entity/.style={rectangle, draw=black!90,  fill=black!20, minimum size=1cm,  text width=1.7cm, font={\Large}, align=center},
                every edge/.append style ={
                                inner sep=0pt, auto,
                                align=left},
                every new --/.style={line width=0.5pt},
        ]
        \node (company) [entity] {\erlcompany};
        \node (person) [entity, right=1.25cm of company] {\erlperson};
        \node (bel_person) [below=of person]{};
        \node (place) [entity, right=2cm of bel_person] {\erlplace};
        \node (school) [entity, right=1.5cm of person] {\erlschool};
        \graph [use existing nodes] {
        company.east --[ out=0,in=180]person.west;
        person.east--[out=0,in=180]place.west;
        person.east--[out=0,in=180]school.west;
        };

\end{tikzpicture}

==> figures/erl_unconstrained.tex <==
\usetikzlibrary {arrows.meta, graphs, shapes.misc, matrix, quotes, patterns, shapes.arrows, shapes.misc, positioning, calc, fit, bending}

\begin{tikzpicture}[
        scale=\erlsize, transform shape,
        entity/.style={rectangle, draw=black!90,  fill=black!20, minimum size=1cm,  text width=1.5cm, font={}, align=center},
        every edge/.append style ={
                inner sep=0pt, auto,
                align=left},
        every new --/.style={line width=0.5pt},
    ]
    \node (company) [entity] {company};
    \node (bel_company) [below=of company]{};
    \node (place) [entity, below=of bel_company] {place};
    \node (person) [entity, left=3cm of bel_company] {person};
    \graph [use existing nodes] {
    person.east--[out=0,in=180, ]company.west;
    person.east--[out=0,in=180]place.west;
    };

\end{tikzpicture}
